CAAT: Contact-Aware Attention Scaling and Tactile Masking for Data-Efficient Contact-Rich Manipulation

In contact-rich manipulation, visual observations primarily guide motion in free space, whereas tactile observations become particularly informative during contact. However, standard Transformer-based visuo-tactile policies typically rely on either token concatenation or learnable gating. These approaches lack explicit contact-aware priors, making it difficult to efficiently learn effective cross-modal representations from demonstrations. To address this limitation, we propose CAAT, a lightweight contact-aware framework that explicitly incorporates contact priors through attention scaling and dynamic tactile masking. Specifically, CAAT emphasizes visual information before contact and tactile information during contact. It also suppresses static background tokens by comparing the current tactile observation with a non-contact reference. CAAT can be integrated into commonly used Transformer-based policies without modifying their action decoders. In simulation, integrating CAAT with ACT improves the average success rate by 18.0 percentage points over direct visuo-tactile fusion and by 10.0 percentage points over gated fusion. In real-world experiments using a visuo-tactile UMI platform, CAAT achieves an average success rate of 60.0% across ACT, Diffusion Policy, and $\pi_0$, outperforming the strongest baseline by an average of 21.1 percentage points. These results demonstrate that explicit contact priors and dynamic tactile masking are effective in improving visuo-tactile policy learning and task performance of diverse policy architectures. https://mrjiangjm.github.io/caat/

==> configs.tex <==
% Common packages
\let\labelindent\relax
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% \usepackage{microtype}
\usepackage{graphicx} \graphicspath{ {figures/} }
\usepackage{amsmath,amssymb}
% ,mathabx,amsbsy,mathtools,etoolbox,mathbbol
\usepackage{times}
\usepackage{graphicx}
\usepackage{algorithmic}
\usepackage[ruled]{algorithm2e}
\usepackage{acronym}
\usepackage{enumitem}
\usepackage{hyperref}
% \usepackage[breaklinks,colorlinks,linkcolor=red,citecolor=blue]{hyperref}
% \usepackage{balance}
\usepackage{xspace}
\usepackage{setspace}
\usepackage[skip=3pt,font=small]{subcaption}
\usepackage[skip=3pt,font=small]{caption}
\usepackage[dvipsnames,svgnames,x11names]{xcolor}
\usepackage[capitalise,nameinlink]{cleveref}
\usepackage{booktabs,tabularx,colortbl,multirow,multicol,array,makecell}
\usepackage{cuted}
\usepackage{capt-of}
% \usepackage{overpic,wrapfig}
% \usepackage{dblfloatfix}
\usepackage[misc]{ifsym}
\usepackage{pifont}
\usepackage{cite}
\usepackage{listings}
\usepackage{anyfontsize}
\usepackage{tikz}
\usepackage{tcolorbox}
\usepackage{booktabs}

% change the reference style
\renewcommand{\citepunct}{,\penalty\citepunctpenalty\,}
\renewcommand{\citedash}{--}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=0.6pt] (char) {#1};}}


% draw a frame around given text
\newcommand{\framedtext}[1]{%
\par\vspace{1mm} % Adds space after the box
\noindent\fbox{%
    \parbox{\dimexpr\linewidth-2\fboxsep-2\fboxrule}{#1}%
}%
\par\vspace{2mm} % Adds space after the box
}

\makeatletter
\AddToHook{cmd/appendix/before}{\def\cref@section@alias{appendix}\def\cref@subsection@alias{appendix}}
\makeatother

% \newenvironment{prompt}
% {\begin{tcolorbox}[colback=gray!5,colframe=gray!40,title=Prompt]}
% {\end{tcolorbox}}


% Handy shorthand
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\eg{\emph{e.g}\onedot} 
\def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} 
\def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{c.f}\onedot} 
\def\Cf{\emph{C.f}\onedot}
\def\etc{\emph{etc}\onedot} 
\def\vs{\emph{vs}\onedot}
\def\aka{a.k.a\onedot}
\def\wrt{w.r.t\onedot} 
\def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}
\makeatother

% Spacing
% \frenchspacing
% % \medmuskip=2mu   % reduce spacing around binary operators
% % \thickmuskip=3mu % reduce spacing around relational operators
% % \setlength{\abovedisplayskip}{6pt}
% % \setlength{\belowdisplayskip}{6pt}
% % \setlength{\abovecaptionskip}{6pt}
% % \setlength{\belowcaptionskip}{6pt}
% \setlength\floatsep{0.5\baselineskip plus 3pt minus 2pt}
% \setlength\textfloatsep{0.5\baselineskip plus 3pt minus 2pt}
% \setlength\dbltextfloatsep{0.5\baselineskip plus 3pt minus 2pt}
% \setlength\intextsep{0.5\baselineskip plus 3pt minus 2pt}

% Handy math ops
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\kl}{KL}
\newcommand\energy{\mathcal{E}}
\newcommand{\norm}[1]{\left\Vert #1 \right\Vert}

\makeatletter
\def\BState{\State\hskip-\ALG@thistlm}
\makeatother

\makeatletter
\renewcommand{\paragraph}{%
  \@startsection{paragraph}{4}%
  {\z@}{0ex \@plus 0ex \@minus 0ex}{-1em}%
  {\hskip\parindent\normalfont\normalsize\bfseries}%
}
\makeatother

\makeatletter
\AtBeginDocument
 {
   \def\ltx@label#1{\cref@label{#1}}%add braces
   \def\label@in@display@noarg#1{\cref@old@label@in@display{#1}}%remove braces
\def\label@in@mmeasure@noarg#1{%
    \begingroup%
      \measuring@false%
      \cref@old@label@in@display{#1}%remove braces for multline, see https://tex.stackexchange.com/q/737204/2388
    \endgroup}%  
 } %
\makeatother

% Clever references
\crefname{algorithm}{Alg.}{Algs.}
\Crefname{algocf}{Algorithm}{Algorithms}
\crefname{section}{Sec.}{Secs.}
\Crefname{section}{Section}{Sections}
\crefname{table}{Tab.}{Tabs.}
\Crefname{table}{Table}{Tables}
\crefname{figure}{Fig.}{Figs.}
\crefname{equation}{Eq.}{Eqs.}
\Crefname{equation}{Equation}{Equations}
\Crefname{figure}{Figure}{Figures}
\crefname{appendix}{Appendix}{Appendices}
\Crefname{appendix}{Appendix}{Appendices}
% \newcommand{\theHalgorithm}{\arabic{algorithm}}

% Handy Colors
\definecolor{gblue}{HTML}{4285F4}
\definecolor{gred}{HTML}{DB4437}
\definecolor{ggreen}{HTML}{0F9D58}
\def\ra{{\color{gblue}R1}}
\def\rb{{\color{gred}R2}}
\def\rc{{\color{ggreen}R3}}
\definecolor{mygray}{gray}{.92}


% Acronym
\acrodef{dof}[DoF]{Degree of Freedom}
\acrodef{vkc}[VKC]{Virtual Kinematic Chain}
\acrodef{tamp}[TAMP]{Task and Motion Planning}
\acrodef{pddl}[PDDL]{Planning Domain Definition Language}
\acrodef{rddl}[RDDL]{Relational Dynamic Influence Diagram Language}
\acrodef{htn}[HTN]{Hierarchical Task Network}
\acrodef{rrt}[RRT]{Rapidly-exploring Random Tree}
\acrodef{ompl}[OMPL]{Open Motion Planning Library}
\acrodef{iws}[IWS]{Iterated Width Search}
\acrodef{bfs}[BFS]{Breadth First Search}
\acrodef{ai}[AI]{Artificial Intelligence}
\acrodef{spt}[SPT]{Scene Parse Tree}
\acrodef{com}[CoM]{Center of Mass}
\acrodef{mcmc}[MCMC]{Markov Chain Monte Carlo}
\acrodef{ged}[GED]{Graph Editing Distance}
% \acrodef{cg}[$cg$]{\textit{Contact Graph}}
% \acrodef{cg+}[$cg^+$]{\textit{Contact Graph}$^+$}
\acrodef{ga}[GA]{Genetic Algorithm}
\acrodef{sgd}[SGD]{Stochastic Gradient Descent}
\acrodef{llm}[LLM]{Large Language Model}
\acrodef{cg}[$cg$]{contact graph}
\acrodef{cga}[$cg^\oplus$]{augmented contact graph}
\acrodef{sdf}[SDF]{Signed Distance Field}
\acrodef{minlp}[MINLP]{mixed-integer nonlinear program}
\acrodef{cmaes}[CMA-ES]{Covariance Matrix Adaptation Evolution Strategy}
\acrodef{vla}[VLA]{Vision-Language-Action}
\acrodef{vqvae}[VQ-VAE]{Vector Quantized Variational Autoencoder}
\acrodef{vae}[VAE]{Variational Autoencoder}
\acrodef{vbts}[VBTS]{Vision-based Tactile Sensor}
\acrodef{act}[ACT]{Action Chunking with Transformers}

\newcommand{\modelname}{TaF-VLA\xspace}

\newcommand{\revision}[1]{{\color{PineGreen}\emph{#1}}}


